WavMark: Watermarking for Audio Generation

Recent breakthroughs in zero-shot voice synthesis have enabled imitating a speaker's voice using just a few seconds of recording while maintaining a high level of realism. Alongside its potential benefits, this powerful technology introduces notable risks, including voice fraud and speaker impersonation. Unlike the conventional approach of solely relying on passive methods for detecting synthetic data, watermarking presents a proactive and robust defence mechanism against these looming risks. This paper introduces an innovative audio watermarking framework that encodes up to 32 bits of watermark within a mere 1-second audio snippet. The watermark is imperceptible to human senses and exhibits strong resilience against various attacks. It can serve as an effective identifier for synthesized voices and holds potential for broader applications in audio copyright protection. Moreover, this framework boasts high flexibility, allowing for the combination of multiple watermark segments to achieve heightened robustness and expanded capacity. Utilizing 10 to 20-second audio as the host, our approach demonstrates an average Bit Error Rate (BER) of 0.48\% across ten common attacks, a remarkable reduction of over 2800\% in BER compared to the state-of-the-art watermarking tool. See https://aka.ms/wavmark for demos of our work.

==> tables/1_shift_compare.tex <==
% \usepackage{multirow}
% \usepackage{booktabs}


\begin{table}[th]
	\centering
%\begin{tabular}{c|c|cccc} 
%	\toprule
%	\multirow{2}{*}{Works} & \multirow{2}{*}{EUL} & \multicolumn{4}{c}{BER(\%) in different shift length}  \\
%	&                      & No & 0.1ms & 1ms & 100ms                               \\ 
%	\hline
%	DeepDNN                & 2.0s                   & 0  & 25    & 43  & 59                                  \\
%	DeAR                   & 11.3s                  & 0  & 0     & 17  & 49                                  \\
%	Ours                   & 1.0s                   & 0  & 0     & 0   & 0                                   \\
%	\bottomrule
%\end{tabular}
%\begin{tabular}{ccccccc} 
%	\toprule
%	\multirow{2}{*}{Works} & \multirow{2}{*}{EUL} & \multicolumn{5}{l}{BER(\%) in different  offset (\%EUL) }  \\ 
%	\cline{3-7}
%	&                      & 0 &   0.001 &   0.01 &   0.1 &   10                                \\ 
%	\hline
%	DeepDNN                & 2s                   & 0.0 &     0.0 &    3.0 &  36.3 & 40.4                             \\
%	DeAR                   & 11s                  &  0.0 &     0.4 &   29.2 &  50.4 & 49.7                      \\
%%	Ours                   & 1s                   &     0.0 &     0.0 &    0.0 &   0.0 &  0.6                                     \\
%	\bottomrule
%\end{tabular}
\begin{tabular}{cccccc} 
	\toprule
	\multirow{2}{*}{Works} & \multirow{2}{*}{EUL} & \multicolumn{4}{l}{BER(\%) in different  offset (\%EUL)}  \\ 
	\cline{3-6}
	&                      & No Offset & 0.001 & 0.01 & 0.1                            \\ 
	\hline
	DeepDNN                & 2s                   & 0.0       & 0.0   & 3.0  & 36.3                           \\
	DeAR                   & 11s                  & 0.0       & 0.4   & 29.2 & 50.4                           \\
	\bottomrule
\end{tabular}
	\caption{
		The existing models have stringent accuracy requirements for locating the watermark position.
		Even a small deviation can lead to a sharp decrease in performance. 
		The term "EUL" refers to the encoding unit length, which represents the length of a watermark section.
	} 
	\label{tab:main_dataset}
	
	%		Decoding performance when the decoded position offset the watermark position.
	%		EUL: encode unit length.
	%现有模型对水印位置存在极高的准确性要求，当解码位置与水印位置存在小范围偏移时，模型性能急剧下降。
	
	%	以往的工作当解码位置发生小范围偏移时性能将急剧下降。	相反，我们的工作获得了对偏移的鲁棒性，即使在100ms偏移下（10\%的位置移动，相对于1s的总编码区域长度），
	%	我们的模型依旧能够成功解码。这使得我们的模型能够适用于剪切攻击与不精确位置解码。
\end{table}

==> tables/2_DeAR_compare.tex <==
\begin{table*}[t]
	\centering
	\begin{tabular}{lccccccccccccc} 
		\toprule
		\multirow{2}{*}{Works} & \multirow{2}{*}{BPS}  & \multirow{2}{*}{SNR} & \multirow{2}{*}{PESQ} & \multicolumn{10}{l}{BER(\%)}                                                                               \\ 
		\cline{5-14}
		&                       &                      &                       & no attack & noise  & bp & resample & mp3    & crop & top & recount & medfilt & record  \\ 
		\hline
		DeAR                   & \multicolumn{1}{r}{9} &                      & 3.55                  & 0.00    & 4.57 & 0.07    & 0.00   & 2.38 & 0.00    & 0.00      & 2.12  & 0.00  & 1.21  \\
		Ours                   & \multicolumn{1}{r}{9} &                      & 4.16                  & 0.00    & 1.67 & 0.00    & 0.00   & 1.53 & 0.00    & 0.00      & 0.97  & 0.00  & 0.14  \\
		\bottomrule
	\end{tabular}
	\caption{
	} 
	\label{tab:comare_DeAR}
\end{table*}

==> tables/3_DNN_compare.tex <==
\begin{table*}[t]
	\centering
\begin{tabular}{ccccccccl} 
	\toprule
	\multirow{2}{*}{Works} & \multirow{2}{*}{BPS} & \multirow{2}{*}{PESQ} & \multirow{2}{*}{SNR} & \multicolumn{5}{l}{BER(\%)}                                                                                                                 \\ 
	\cline{5-9}
	&                      &                       &                      & no attack                 & noise                     & low pass                  & dropout                   & noise + low pass + dropout  \\ 
	\hline
	DNN                    & 1.3                  & 4.21                  & 35.19                &                           &                           &                           &                           &                             \\
	Ours                   & 2.5                  &                       & \multicolumn{1}{l}{} & \multicolumn{1}{r}{0.00~} & \multicolumn{1}{r}{0.00~} & \multicolumn{1}{r}{0.00~} & \multicolumn{1}{r}{0.00~} & \multicolumn{1}{r}{0.00~}   \\
	\bottomrule
\end{tabular}
	\caption{
	} 
	\label{tab:comare_DNN}
\end{table*}

==> tables/4_my_attack_compare.tex <==
\begin{table*}[t]
%	todo：起始不一定要重新finetune别的，大不了注明一下是在他们自己的数据集上用哪些攻击测试出来的效果
	\centering
\begin{tabular}{lrlllllllllll} 
	\toprule
	\multicolumn{1}{c}{\multirow{2}{*}{}} & \multicolumn{1}{c}{\multirow{2}{*}{BPS}} & \multicolumn{1}{c}{\multirow{2}{*}{SNR}} & \multicolumn{1}{c}{\multirow{2}{*}{PESQ}} & \multicolumn{9}{l}{BER(\%)}                                                                    \\ 
	\cline{5-13}
	\multicolumn{1}{c}{}                  & \multicolumn{1}{c}{}                     & \multicolumn{1}{c}{}                     & \multicolumn{1}{c}{}                      & no attack & noise & dropout & low pass & MF & mp3 & resample & CS & echo  \\ 
	\hline
	DNN                                   & 1.3                                      &                                          &                                           &           &       &         &          &               &     &          &              &       \\
	DeAR                                  & 8.8                                        &                                          &                                           &           &       &         &          &               &     &          &              &       \\
	Patch2017                             & 10                                       &                                          &                                           &           &       &         &          &               &     &          &              &       \\
	De2021                                & 30                                       &                                          &                                           &           &       &         &          &               &     &          &              &       \\
	Ours (-S)                         & 2.5                                       &                                          &                                           &           &       &         &          &               &     &          &              &       \\
	Ours (-S)                         & 10                                       &                                          &                                           &           &       &         &          &               &     &          &              &       \\
	Ours (-S)                         & 32                                       &                                          &                                           &           &       &         &          &               &     &          &              &       \\
	Ours                                  & 32                                       &                                          &                                           &           &       &         &          &               &     &          &              &       \\
	\bottomrule
\end{tabular}
	\caption{
	} 
	\label{tab:my_attack_compare}
\end{table*}

==> tables/5_my_attack_compare_slim.tex <==
\begin{table*}[t]
	\centering
\begin{tabular}{cl|llllll} 
	\toprule
	\multicolumn{2}{c|}{Metrics}              & DeAR                  & Patch2017              & De2021                 & Ours-v1                & Ours-v2                & Ours-v2+SI              \\ 
	\hline
	\multicolumn{2}{l|}{capacity（bps）}        & \multicolumn{1}{r}{9} & \multicolumn{1}{r}{10} & \multicolumn{1}{r}{30} & \multicolumn{1}{r}{10} & \multicolumn{1}{r}{30} & \multicolumn{1}{r}{30}  \\
	\multicolumn{2}{l|}{SNR (db)}             &                       &                        &                        &                        &                        &                         \\
	\multicolumn{2}{l|}{PESQ}                 &                       &                        &                        &                        &                        &                         \\
	\multirow{12}{*}{BER(\%)} & no-attack     &                       &                        &                        &                        &                        &                         \\
	& random noise  &                       &                        &                        &                        &                        &                         \\
	& dropout       &                       &                        &                        &                        &                        &                         \\
	& low pass      &                       &                        &                        &                        &                        &                         \\
	& medium filter &                       &                        &                        &                        &                        &                         \\
	& mp3 codec     &                       &                        &                        &                        &                        &                         \\
	& down sample   &                       &                        &                        &                        &                        &                         \\
	& up sample     &                       &                        &                        &                        &                        &                         \\
	& up speed      &                       &                        &                        &                        &                        &                         \\
	& down speed    &                       &                        &                        &                        &                        &                         \\
	& echo addtion  &                       &                        &                        &                        &                        &                         \\
	& random shift  &                       &                        &                        &                        &                        &                         \\
	\bottomrule
\end{tabular}
	\caption{
	} 
	\label{tab:my_dataset_compare}
\end{table*}

==> tables/7_DeAR_DNN_compare_v0.tex <==
\begin{table*}[th]
	\centering
	\resizebox{1.0\columnwidth}{!}{%
\begin{tabular}{lrrrrrrrlllllr} 
	\toprule
	\multirow{2}{*}{Models} & \multicolumn{1}{c}{\multirow{2}{*}{BPS(↑)}} & \multicolumn{1}{c}{\multirow{2}{*}{SNR(↑)}} & \multicolumn{1}{c}{\multirow{2}{*}{PESQ(↑)}} & \multicolumn{9}{l}{BER(\%)(↓)}                                                                                                                                                                                                                                       &                         \\
	& \multicolumn{1}{c}{}                        & \multicolumn{1}{c}{}                        & \multicolumn{1}{c}{}                         & \multicolumn{1}{c}{No Attack} & \multicolumn{1}{c}{RN} & \multicolumn{1}{c}{LP} & \multicolumn{1}{c}{SS} &                                   &                           &                           &                                   &                           & \multicolumn{1}{l}{}    \\ 
	\hline
	RobustDNN              & 1.2                                         & 26.9                                        & 4.17                                        & 0.00                         & 0.00                  & 0.00                  & 0.49                  &                                   &                           &                           &                                   &                           & \multicolumn{1}{l}{}    \\
	Ours-2.5bps             & \textbf{2.5}                                & \textbf{41.2}                               & \textbf{4.31}                                & 0.00                         & 0.00                  & 0.00                 & \textbf{0.00}                  &                                   &                           &                           &                                   &                           & \multicolumn{1}{l}{}    \\[5pt]
	& \multicolumn{1}{l}{}                        & \multicolumn{1}{l}{}                        & \multicolumn{1}{l}{}                         & \multicolumn{1}{c}{No Attack} & \multicolumn{1}{c}{RN} & \multicolumn{1}{c}{BP} & \multicolumn{1}{c}{RS} & \multicolumn{1}{c}{LC}            & \multicolumn{1}{c}{DO}    & \multicolumn{1}{c}{CA}    & \multicolumn{1}{c}{QTZ}           & \multicolumn{1}{c}{MF}    & \multicolumn{1}{c}{RD}  \\
	DeAR                   & 8.8                                         & 25.00                                     & 3.55                                        & 0.00                         & 4.57                  & 0.07                  & 0.00                  & \multicolumn{1}{r}{2.38}         & \multicolumn{1}{r}{0.00} & \multicolumn{1}{r}{0.00} & \multicolumn{1}{r}{2.12}         & \multicolumn{1}{r}{0.00} & 1.21                   \\
	Ours-9bps               & \textbf{9.0}                                & \textbf{31.57}                              & \textbf{4.16}                                & 0.00                         & \textbf{1.67}          & \textbf{0.00}                 & 0.00                  & \multicolumn{1}{r}{\textbf{1.53}} & \multicolumn{1}{r}{0.00} & \multicolumn{1}{r}{0.00} & \multicolumn{1}{r}{\textbf{0.97}} & \multicolumn{1}{r}{0.00} & \textbf{0.14}           \\
	\bottomrule
\end{tabular}
}
	\caption{
Comparison with previous DNN-based methods.
The scores of the compared models were obtained from the authors' released models.
The attacks  are from the compared works, and more details can be found in papers~\cite{DNN2022DSP,DeAR2023AAAI}.
BP: Band Pass. DO: Dropout. RD: Re-recording.
		 } 
	\label{tab:comare_DeAR_DNN22}
\end{table*}

==> tables/7_DeAR_DNN_compare_v1.tex <==
\begin{table*}[th]
	\centering
	\resizebox{1.0\columnwidth}{!}{%
\begin{tabular}{lrrrrrrrrrrrrrrr} 
	\toprule
	\multicolumn{1}{c}{\multirow{2}{*}{Models}} & \multicolumn{1}{c}{\multirow{2}{*}{BPS(↑)}} & \multicolumn{1}{c}{\multirow{2}{*}{SNR(↑)}} & \multicolumn{1}{c}{\multirow{2}{*}{PESQ(↑)}} & \multicolumn{12}{l}{BER(\%)(↓)}                                                                                                                                                                                                                                   \\
	\multicolumn{1}{c}{}                        & \multicolumn{1}{c}{}                        & \multicolumn{1}{c}{}                        & \multicolumn{1}{c}{}                         & NoAttack & RN    & LP                    & SS                    & BP                    & RS                    & LC                    & DO                    & CA                    & QTZ                   & MF                    & RD                     \\ 
	\hline
	RobustDNN                                   & 1.2                                         & 26.90~                                      & 4.17                                         & 0.00~    & 0.00~ & 0.00~                 & 0.49~                 & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-}  \\
	Ours-2.5bps                                 & 2.5                                         & 41.20~                                      & 4.31                                         & 0.00~    & 0.00~ & 0.00~                 & 0.00~                 & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-}  \\
	& \multicolumn{1}{l}{}                        & \multicolumn{1}{l}{}                        & \multicolumn{1}{l}{}                         &          &       &                       &                       &                       &                       &                       &                       &                       &                       &                       &                        \\
	DeAR                                        & 8.8                                         & 25.00~                                      & 3.55                                         & 0.00~    & 4.57~ & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & 0.07~                 & 0.00~                 & 2.38~                 & 0.00~                 & 0.00~                 & 2.12~                 & 0.00~                 & 1.21~                  \\
	Ours-9bps                                   & 9                                           & 31.57~                                      & 4.16                                         & 0.00~    & 1.67~ & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & 0.00~                 & 0.00~                 & 1.53~                 & 0.00~                 & 0.00~                 & 0.97~                 & 0.00~                 & 0.14~                  \\
	& \multicolumn{1}{l}{}                        & \multicolumn{1}{l}{}                        & \multicolumn{1}{l}{}                         &          &       &                       &                       &                       &                       &                       &                       &                       &                       &                       &                        \\
	Ours-32bps                                  & 32                                          & 39.98~                                      & 4.35                                         & 0.30~    & 1.17~ & 1.08~                 & \multicolumn{1}{c}{-} & \multicolumn{1}{c}{-} & 1.15~                 & 0.70~                 & 0.87~                 & 0.32~                 & 1.96~                 & 5.86~                 & \multicolumn{1}{c}{-}  \\
	\bottomrule
\end{tabular}
}
	\caption{
Comparison with previous DNN-based methods.
The scores of the compared models were obtained from the authors' released models.
The attacks  are from the compared works, and more details can be found in papers~\cite{DNN2022DSP,DeAR2023AAAI}.
BP: Band Pass. DO: Dropout. RD: Re-recording.
		 } 
	\label{tab:comare_DeAR_DNN22}
\end{table*}

==> tables/8_compare_on_5s_dataset_v1.tex <==
\begin{table*}[th]
	\centering
%\begin{tabular}{clllllllll} 
%	\toprule
%	\multirow{2}{*}{Location} & \multicolumn{9}{l}{BER(\%)}                                                                    \\
%	& no attack & noise & dropout & low pass & medium filter & mp3 & resample & change speed & echo  \\ 
%	\hline
%	Oracle                       &           &       &         &          &               &     &          &              &       \\
%	BFD                      &           &       &         &          &               &     &          &              &       \\
%	\bottomrule
%\end{tabular}

\begin{tabular}{lrrlrrrrrrrrrr} 
	\toprule
	\multicolumn{1}{c}{\multirow{2}{*}{Shift Module}} & \multicolumn{1}{c}{\multirow{2}{*}{SNR}} & \multicolumn{1}{c}{\multirow{2}{*}{PESQ}} & \multirow{2}{*}{Locating} & \multicolumn{10}{l}{BER(\%)}                                                       \\
	\multicolumn{1}{c}{}                        & \multicolumn{1}{c}{}                     & \multicolumn{1}{c}{}                      &                           & No attack & RN    & SS    & LP    & MF    & MP3   & QTZ    & RS    & TS    & EA   \\ 
	\hline
	\multirow{2}{*}{w/o SM}                      & \multirow{2}{*}{0.00}                    & \multirow{2}{*}{0.00}                     & Oracle                    & 0.20 &    0.36 &      0.75 &       0.44 &            4.71 &  1.23 &           2.85 &       0.67 &           1.62 &   0.32 \\
	
	
	&                                          &                                           & SyncCode                  & 6.96 &    7.17 &      7.81 &      15.30 &           16.88 & 10.34 &           9.81 &      15.66 &          41.14 &   7.81 \\[5pt]
	
	
	
	\multirow{2}{*}{w SM}                      & \multirow{2}{*}{38.75}                   & \multirow{2}{*}{4.40}                     & Oracle                    &0.24 &    4.71 &      0.83 &       0.87 &            6.92 &  1.19 &           7.44 &       1.15 &           4.67 &   0.44 \\
	
	
	&                                          &                                           & BFD                       &0.11 &    4.96 &      0.53 &       0.84 &            8.44 &  1.27 &           5.70 &       1.37 &           7.38 &   0.74 \\
	\bottomrule
\end{tabular}
	\caption{Comparison of different watermark localization schemes.} 
	\label{tab:comare_oracle_bdf}
\end{table*}
